Addressing pitfalls in implicit unobserved confounding synthesis using explicit block hierarchical ancestral sampling

Unbiased data synthesis is crucial for evaluating causal discovery algorithms in the presence of unobserved confounding, given the scarcity of real-world datasets. A common approach, implicit parameterization, encodes unobserved confounding by modifying the off-diagonal entries of the idiosyncratic covariance matrix while preserving positive definiteness. Within this approach, we identify that state-of-the-art protocols have two distinct issues that hinder unbiased sampling from the complete space of causal models: first, we give a detailed analysis of use of diagonally dominant constructions restricts the spectrum of partial correlation matrices; and second, the restriction of possible graphical structures when sampling bidirected edges, unnecessarily ruling out valid causal models. To address these limitations, we propose an improved explicit modeling approach for unobserved confounding, leveraging block-hierarchical ancestral generation of ground truth causal graphs. Algorithms for converting the ground truth DAG into ancestral graph is provided so that the output of causal discovery algorithms could be compared with. We draw connections between implicit and explicit parameterization, prove that our approach fully covers the space of causal models, including those generated by the implicit parameterization, thus enabling more robust evaluation of methods for causal discovery and inference.

==> a_google_doc.tex <==
https://docs.google.com/document/d/1IX0WsPCGvWmMxhUJQbSCYbIJV8tfLGPoSE3quGB8yeM/edit?usp=sharing

==> abandoned.tex <==
\begin{align}
	%&f^{\dagger}
	 & \text{causal discovery}\colon D \sim \mathbb{D} \to (O)MEC(\mathbb{G}) \\
	 & \text{causalspyne} \colon \mathbb{G} \to \mathbb{P} \to \mathbb{D}
\end{align}

==> figs_ancestral_vs_fci.tex <==
\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
\includegraphics[width=0.95\linewidth]{figs/figs_temp/graph_compare_20241103_110540_dags_percentil0.pdf}
        \caption{Example DAG generated via our new data generation process and the corresponding ancestral ADMG when hiding the root variable $X0$ (To conform to FCI output, we put $X$ in front of node index).}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
\includegraphics[width=0.85\linewidth]{figs/figs_temp/output_causallearn_graph_compare_20241031_154418_dags_hide_root.png}
        \caption{FCI output when feeding FCI with data missing column $X0$.}
    \end{subfigure}
\caption{The ground truth ancestral ADMG has several bidirected edges, FCI at least managed to identify a portion of the arrow heads correctly.}\label{fig:dag2ancestra_vs_fci_root}
%Source code: \url{https://github.com/marrlab/causalspyne}, percentile=[0]
\end{figure}


\begin{figure}
  \begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/figs_temp/graph_compare_20241103_110926_dags_percentil_07_09.pdf}
\caption{Example DAG generated via our new data generation process and the corresponding ancestral ADMG when hiding intermediate confounder $X2, X5$ (To conform to FCI output, we put $X$ in front of node index).}
\end{subfigure}
\begin{subfigure}[b]{0.48\textwidth}
\centering
\includegraphics[scale=0.25]{figs/figs_temp/output_causallearn_graph_compare_20241031_155020_dags._hidep0907.png}
\caption{FCI output when feeding FCI with data missing column $X2, X5$.}
\end{subfigure}
\caption{There is no bidirected edge in the ground truth ancestral ADMG, but FCI falsely identified many bidirected edges.}\label{fig:dag2ancestra_vs_fci_intermediate}
\end{figure}




==> marginal_abstraction_and_confounders_copyPratik.tex <==
\subsection{marginal abstraction and confounders}
In this section, we compare the marginal Gaussian distributions on the observed variables obtained before and after marginalizing out certain variables and adding appropriate confounders. Let $X=(X_1,\ldots,X_n)$ be a random vector and $f(x)$ be its probability distribution function. Then the recursive factorization property of graphical models is that
the conditional densities $f_i(x_i|x_1,\ldots,x_{i-1})$ only depends on the parents of $i$, i.e., $f_i(x_i|x_1,\ldots,x_{i-1})=f_i(x_i|x_{pa(i)})$. For a Gaussian DAG model, this recursive factorization allows us to write the covariances in terms of treks in $G$. We use the trek rule expression in the remainder of the section to make the comparison between the models.

For a given DAG $G$, marginalizing a vertex $i$ corresponds to deleting the vertex from the DAG and producing a mixed graph which preserves the causal relations among all the other variables. Let $G\setminus i$ denote the subgraph induced by $G$ on $V(G)\setminus i$ nodes.  The following rule is followed to construct the mixed graph after marginalization:
\begin{itemize}
    \item If $i$ is a sink node, the mixed graph is exactly the subgraph $G\setminus i$.
    \item If $j$ is a parent of $i$ and $k$ is a child of $i$, then the corresponding mixed graph is obtained by adding directed edges from $j$ to $k$ in $G\setminus i$.
    \item If $i$ has more than child, say $k$ and $l$, then corresponding mixed graph is obtained by adding bidirected edges between $k$ and $l$ in $G\setminus i$.
\end{itemize}

Now, the only interesting case in this setup is the case where we obtain a bidirected edge. This is because different DAGs can end up producing the same mixed graph upon marginalization. The most general DAG that can be reconstructed from a mixed graph is one where every bidirected edge $k\leftrightarrow l$ is replaced by a new vertex $i$ along with the directed edges $i\rightarrow k$ and $i\rightarrow l$. We denote this new DAG by $G'$. Although $G$ and $G'$ satisfy the same set of polynomial constraints among the covariances of the observed variables, they could still differ as models. For instance, there could be certain polynomial inequalities (semi-algebraic constraints) that are satisfied by one of the DAGs and not by the other. We illustrate this with an example.

\begin{example}
Let $G$ be the DAG on 4 nodes with the edge set $\{1\rightarrow 2, 1\rightarrow 3, 1\rightarrow 4\}$. Upon marginalization of the vertex $1$, we obtain the mixed graph with vertices $2,3,4$ and bidirected edges $\{2\leftrightarrow 3, 2\leftrightarrow 4, 3\leftrightarrow 4\}$. Now, in order to obtain $G'$, we add 3 new confounders $1,5$ and $6$, so that we get the DAG on 6 vertices with the edge set $\{1\rightarrow 2, 1\rightarrow 3, 5\rightarrow 3, 5\rightarrow 4, 6\rightarrow 2, 6\rightarrow 4\}$. Both DAGs do not satisfy any polynomial constraints in the covariances of the observed variables $2,3$ and $4$. Using the trek rule on $G$, we can explicitly state the covariances in terms of the error variances $\omega$ and structural coefficients $\lambda$ in the following way:
\begin{eqnarray*}
\sigma_{23}&=&\omega_1\lambda_{12}\lambda_{13} \\    
\sigma_{24}&=&\omega_1\lambda_{12}\lambda_{14} \\
\sigma_{34}&=&\omega_1\lambda_{13}\lambda_{14}.
\end{eqnarray*}
Similarly, for $G'$, we get:
\begin{eqnarray*}
\sigma_{23}&=&\omega_1\lambda_{12}\lambda_{13} \\    
\sigma_{24}&=&\omega_6\lambda_{62}\lambda_{64} \\
\sigma_{34}&=&\omega_5\lambda_{53}\lambda_{54}.
\end{eqnarray*}
As all the error variances are non-negative, we get the following inequality constraint for $G$
\[
\sigma_{23}\sigma_{24}\sigma_{34}= \omega_1^3\lambda_{12}^2\lambda_{13}^2\lambda_{14}^2 \geq 0,
\]
which is not necessarily true for $G'$ as 
\[
\sigma_{23}\sigma_{24}\sigma_{34}= \omega_1 \omega_5 \omega_6 \lambda_{12}\lambda_{13}\lambda_{62}\lambda_{64}\lambda_{53}\lambda_{54},
\]
could be negative for certain choice of the structural coefficients.
\end{example}

The above example shows that the corresponding models might differ even though they satisfy the same constraints on the covariances of the observed variables. We do however, conjecture that even though the two models are different, the model obtained from $G$ is always contained in the one obtained from $G'$. This is because, one could potentially assign specific values to certain variance and edge parameters of $G'$ to obtain the exact same parametrization as $G$. For instance, in the above example, we could set 
\begin{eqnarray*}
\omega_1^{G'}=\omega_5^{G'}=\omega_6^{G'}=\omega_1^G \text{ and} \\
\lambda_{62}^{G'}=\lambda_{12}^G, \lambda_{53}^{G'}=\lambda_{13}^G, \\
\lambda_{54}^{G'}=\lambda_{64}^{G'}=\lambda_{14}^G
\end{eqnarray*}
to obtain the same parametrization of $G$.

\begin{todo}
This implies even if the two DAGs discussed here are O-Markov equivalent, i.e., the set of CIs w.r.t. only observables are the same. Their parametrization can be different, one satisfy an algebraic constraint, another not. But still, it is not possible to distinguish the two different parametrization from observed data?   Does this have a connection to arid ADMG and bow-free ADMG at all?  (ancestral ADMG $\subset$ arid ADMG 
$\subset$ Bow free ADMG. 
\end{todo}
%\end{document}

==> metric.tex <==
\subsection{Evaluation Metric}
\begin{itemize}
	\item ancestral accuracy: for each pair of observed variable $(u,v)$, no matter if an edge exist or not, we can evaluate whether their ancestral relationship is being predicted correctly or not.
	      If there are $m_{obs}$ a number of observed variables, then $\frac{m_{obs}(m_{obs}-1)}{2}$ the number of ancestral relationships need to be compared between ground truth and prediction.
\end{itemize}


==> proof_one_plus_explicit_pd.tex <==
\begin{proof}\label{proof:1plusexplicit_always_psd}
	Let $\xi$ be as in \Cref{prop:explicit_always_psd} with i.i.d.\ components such that $\operatorname{var}(\xi_i)=1$, and suppose $\epsilon_O$ is also i.i.d.\ with $\operatorname{var}(\epsilon_i)=1$.

	When $|J_U|=1$, $\Lambda$ is a column vector and the resulting outer product yields
	\[
		\Omega_{i,j} = [\Lambda\Lambda^T]_{ij} + \delta_{i,j} = \Lambda_{i}\Lambda_{j} + \delta_{i,j},
	\]
	which is a special case of~\Cref{eq:explicit_always_psd}.
	By~\Cref{eq:constraint_mat_Lambda}, there exist indices $i^*\neq j^*$ such that $\Lambda_{i^*}\neq0$ and $\Lambda_{j^*}\neq0$.
	This implies that
	\[
		\Omega_{i^*,j^*} = \Lambda_{i^*}\Lambda_{j^*}.
	\]

	If we further choose the off-diagonal entries such that
	\[
		\Omega_{i,j} = \delta_{i,i^*}\delta_{j,j^*}, \quad \text{for } i \neq j,
	\]
	and ensure that $\Lambda_{i^*}$ and $\Lambda_{j^*}$ share the same sign, then we obtain
	\[
		\Omega_{i,i} = 1+\sum_{j\neq i}|\Omega_{j,i}|.
	\]

	For the case of more than one unobserved confounder (i.e., $|J_U|>1$), \Cref{eq:explicit_always_psd} leads to
	\[
		\Omega_{i,j} = [\Lambda\Lambda^T]_{i,j} + \delta_{i,j} = \sum_k \Lambda_{i,k}\Lambda_{j,k} + \delta_{i,j},
	\]
	where the dummy index $k$ iterates over $J_U$.
	Under the assumption that each confounder $k$ only affects one pair of variables and that for each $k$ the corresponding entries $\Lambda_{i,k}$ and $\Lambda_{j,k}$ share the same sign, a similar conclusion follows, namely that
	\[
		\Omega_{i,i} = 1+\sum_{j\neq i}|\Omega_{j,i}|.
	\]
	\todo{XS: this proof is not correct, will fix}
\end{proof}




==> proof_par_corr_exclude_one_var_wrong.tex <==
Now the additive factors of $Y_i^T(I-P_{\setminus i,j} - P_{(I-P_{\setminus i,j})Y_i})(I-P_{\setminus i,j} - P_{(I-P_{\setminus i,j})Y_j})Y_j$:

\begin{align}
&Y_i^TP_{(I-P_{\setminus i,j})Y_i}P_{(I-P_{\setminus i,j})Y_j}Y_j\\
=&Y_i^T\bigl((I-P_{\setminus i,j})Y_i\bigr){\Bigl(Y_i^T(I-P_{\setminus i,j})(I-P_{\setminus i,j})Y_i\Bigr)}^{-1}Y_i^T(I-P_{\setminus i,j})\nonumber\\
 &\bigl((I-P_{\setminus i,j})Y_j\bigr){\Bigl(Y_j^T(I-P_{\setminus i,j})(I-P_{\setminus i,j})Y_j\Bigr)}^{-1}Y_j^T(I-P_{\setminus i,j})Y_j \nonumber\\
=&Y_i^T(I-P_{\setminus i,j})Y_j~\text{(middle factors, rest cancels to identity)}
\end{align}

\begin{align}
&Y_i^T(I-P_{\setminus i,j})P_{(I-P_{\setminus i,j})Y_j}Y_j\\
=&Y_i^T(I-P_{\setminus i,j})\bigl((I-P_{\setminus i,j})Y_j\bigr){\Bigl(Y_j^T(I-P_{\setminus i,j})(I-P_{\setminus i,j})Y_j\Bigr)}^{-1}Y_j^T(I-P_{\setminus i,j})\nonumber\\
 &Y_j\nonumber\\
=&Y_i^T(I-P_{\setminus i,j})Y_j~\text{(first 4 factors, rest cancels to identity)}
\end{align}

\begin{align}
&Y_i^TP_{(I-P_{\setminus i,j})Y_i}(I-P_{\setminus i,j})Y_j\\
=&Y_i^T\bigl((I-P_{\setminus i,j})Y_i\bigr){\Bigl(Y_i^T(I-P_{\setminus i,j})(I-P_{\setminus i,j})Y_i\Bigr)}^{-1}Y_i^T(I-P_{\setminus i,j})\nonumber\\
 &(I-P_{\setminus i,j})Y_j\nonumber\\
=&Y_i^T(I-P_{\setminus i,j})Y_j~\text{(last 4 factors, rest cancels to identity)}
\end{align}
so
\begin{align}
&\hat{\epsilon}^T_{i|i}\hat{\epsilon}_{j|j}\\
=&\hat{\epsilon}_{i|i,j}^T\hat{\epsilon}_{j|i,j} + \hat{\epsilon}_{i|i,j}^T\hat{\epsilon}_{j|i,j} - \\
 &Y_i^T(I-P_{\setminus i,j})P_{(I-P_{\setminus i,j})Y_j}Y_j-Y_i^TP_{(I-P_{\setminus i,j})Y_i}(I-P_{\setminus i,j})Y_j
\end{align}
\todo{XS: the current result is zero, contradict!}



==> proof_partial_corr_single_entry_hillar.tex <==
Since $|{[\Omega^{-1}]}_{i,j}|<{||\Omega^{-1}||}_{\infty}$, take $\rho<1$, s.t.

$0\le\min|{[\Omega^{-1}]}_{i,j}|<\rho^k{||\Omega^{-1}||}_{\infty}<\cdots<\rho^2{||\Omega^{-1}||}_{\infty}<\max|{[\Omega^{-1}]}_{i,j}|<\rho{||\Omega^{-1}||}_{\infty}$ with $\rho<<1$

\begin{equation}
B(V)=\frac{3|V|-4}{2\ell(|V|-2)(|V|-1)}=\frac{3}{2}\frac{|V|-4/3}{\ell(|V|-2)(|V|-1)}>\frac{3}{2\ell}\frac{|V|-4/3}{|V|^2}
\end{equation}

we have $\exists i, j$, s.t.

\begin{align}
  |\rho_{i,j|V/\{i,j\}}|&=\frac{{[\Omega^{-1}]}_{i,j}}{\sqrt{{[\Omega^{-1}]}_{i,i}{[\Omega^{-1}]}_{j,j}}}\\
                        &=<\frac{\rho^k}{B(V)}<\frac{2\rho\ell}{3}\frac{|V|^2}{|V|-4/3}<1
\end{align}
so that the range of the partial correlation does not reach $1$.

%since $1-(1/B(v))^2>1-\frac{4|V|^4}{9(|V|-4/3)^2}$

An example for the test statistic for the partial correlation is
\begin{align}
  t&=\frac{\rho_{i,j|V/\{i,j\}}\sqrt{N-2-(|V|-2)}}{\sqrt{1-\rho_{i,j|V/\{i,j\}}^2}}\\&<\frac{1/B(v)}{\sqrt{1-{(1/B(v))}^2}}\sqrt{N-2-(|V|-2)}\\    
   &=\sqrt{x^2/(1-x^2)}
%   &<\frac{2}{3}\frac{|V|^2}{|V|-4/3}\sqrt{N-2-(|V|-2)}
\end{align} should follow t-distribution with degrees of freedom $N-2-(|V|-2)$ where $N$ is the number of samples.
%%%%%%%%This in general will have more edges being removed during the FCI process. 



==> prop_inverse_trek_rule.tex <==
\begin{proposition}[off-diagonal entries of $\Omega$ in $\Sigma$]
  \begin{align}
    \Omega_{i,j}&=\sum_{k,q}{[(I-W)]}_{i,k}\Sigma_{k,q}{[(I-W)^T]}_{q,j}\\
                &=\Sigma_{i,j}-\sum_k W_{i,k}\Sigma_{k,j}-\sum_k \Sigma_{i,k}W_{j,k}\nonumber\\
    +&\sum_{q_1, q_2} W_{i,q_1}\Sigma_{q_1, q_2}W_{j,q_2}\\
%    W_{i,k}&\neq 0
s.t.~&~(\text{if}~\Omega\in \mathcal{A}_B)\nonumber\\
W_{i,j}&=0\\
{[W^2]}_{i,j}&=\sum_qW_{i,q}W_{q,j}=0\\
&\ldots\nonumber\\
{[W^k]}_{i,j} &= \Sigma_{q_1, q_2, \ldots, q_{k-1}}W_{i,q_1}W_{q_1, q_2}\ldots W_{q_{k-2},q_{k-1}}W_{q_{k-1}, j}=0
  \end{align}
\end{proposition}
\begin{proof}
Inverse congruent transform of~\Cref{eq:corr_y} gives
\begin{align}
        \Omega & :=\mathbb{E}(YY^T) = {(I-W)}\Sigma{({(I-W)}^{-T})}^{-1}\label{eq:corr_y_inv_congruent}\\
               &={(I-W)}\Sigma{({(I-W)}^{T})}\label{eq:corr_y_inv_congruent_simply}\\
               &=\Sigma-W\Sigma-\Sigma W^T+ W\Sigma W^T
\end{align}
where~\Cref{eq:corr_y_inv_congruent_simply} is due to ${({({(I-W)}^{-1})}^T)}^{-1}={({({(I-W)}^{-1})}^{-1})}^T$ by substituting $A=(I-W)$ below.
\begin{align}
  A^T(A^{-1})^T &=  (A^{-1}A)^{T} = I^T = I \\
  (A^{-1})^TA^T &=  (AA^{-1})^{T} = I^T = I
\end{align}


\end{proof}





==> related_work.tex <==
\section{Related work}
\citep{bhattacharya2021differentiable} extends ancestral ADMGs (acyclic directed mixed graph) to general ADMG to incorporate equality restrictions on the observed variable and proposed continuous optimization in the hypothesis space. 


==> sec_work_in_progress.tex <==
\subsection{work in progress (don't read)}
\begin{lemma}
  \begin{equation}
    \begin{bmatrix} 
      &\Sigma_{11} &\Sigma_{12}\\
      &\Sigma_{21} &\Sigma_{22}
    \end{bmatrix}
  \end{equation}
  share the same $\Sigma_{11}$ covariance structure with 
  \begin{equation}
    \begin{bmatrix} 
      &\Sigma_{11} &\Sigma_{12}Q\\
      &Q^T\Sigma_{21} &Q^T\Sigma_{22}Q + R
    \end{bmatrix}
  \end{equation}
where $Q$ is orthogonal, $0\prec R$
since orthgonal transform does not change the norm
\begin{equation}
  ||\Sigma_{12}Q||\le ||\Sigma_{12}
\end{equation}
The Schur complement of $\Sigma_{11}$ in the second covariance matrix is p.s.d.~.

\end{lemma}

\begin{lemma}
The transformation 
\begin{equation}
eigm(\Sigma_2)\sqrt{diag(\lambda(\Sigma_2))}(eigm(\Sigma_1)\sqrt{diag(\lambda(\Sigma_1))})
\end{equation}
  maps variables that result in covariance matrix change.
\end{lemma}

\input{thm_o_markov_equiv}



==> sem_conjecture_hack_diag_dom.tex <==
It turns out we could estimate (upper bound and lower bound) the off-diagonal energy of the $\Omega$ matrix via the special diagonally dominant structure through the following conjecture. %~\Cref{conj:off_diag_energy}.
\input{prop_inverse_trek_rule}
\begin{conjecture}\label{conj:off_diag_energy}
Given $\Sigma, \max_{i,j} W_{i,j}$, via~\Cref{eq:corr_y_inv_congruent}:$\Omega=(I-W)\Sigma{(I-W)}^T$, the spectrum of $\Omega$ could be estimated via Ostrowski's theorem, via extra diagonally dominant constraint of $\Omega$, the spectrum estimation of $\Omega$ can be refined via~\Cref{lemma:spectrum_radius_omega_diag_dom}. 

Note that the eigenvalues of diagnal matrix are simply the diagonal elements themselves with the eigenvector being the standard basis vectors.

Let $diag(\Omega)$ be the diagonal part of $\Omega$, $E$ be the off diagonal part of $\Omega$, according to Weyl's inequality, we have
\begin{align}
  \max_j|\lambda_j({diag(\Omega)}) - \lambda_j({\Omega})| &\le \| E \|_{\text{F}}\\
  \max_j|\Omega_{jj} - \lambda_j({\bf \Omega})| &\le \| E \|_{\text{F}}
\end{align}
where $\| E \|_{\text{F}}$ is the Frobenius norm of $E$.
\end{conjecture}

\begin{conjecture}\label{conj:diag_dom_diag_congruent_inv}
  $\exists D=diag(1, \rho, \ldots, \rho^{|V|-1}), s.t.~\hat{\Omega}=D^T\Sigma D$ from~\Cref{lemma:diag_dom_diag_congruent2non_diag_dom} which diminishes off-diagonal entries but preserves the sparse off-diagonal structure of $\Omega$ via thresholding out small off-diagonal entries via the estimated off-diagnoal energy.
\end{conjecture}



\begin{conjecture}
When expressing the solution of a causal discovery algorithm (e.g.~FCI) to be in the form of $\hat{W}$ and $\hat{\Omega}$ by filling the indeterminant entries (The ground truth ancestral graph only has directed and bidirected edges, but e.g.~FCI returns a partial ancestral graph with undirected edges) to satisfy the p.s.d.~constraint, corresponding to the estimated value for~\Cref{eq:wplp}, the corresponding $\hat{\Omega}$ does \textbf{NOT} necessarily lies in the constrained p.s.d.~space specified by~\Cref{coro:omega_psd}.
\end{conjecture}


==> spirtes02.tex <==
\subsection{CI and parametrization connection}
\begin{todo}
\citet{spirtes2002} in section 8.3.1 shows a non-maximal ancestral graph offers only a subset of distributions.
\citet{spirtes2002} in section 8.6 gives a counter example when the \textbf{canonical} DAG corresponding to a 3-nodes complete ancestral ADMG can not parameterize all distributions.
Prop8.6 before 8.1.3 subgraph contains
\end{todo}


==> thm_o_markov_equiv.tex <==
\begin{myconjecture}
	\label[myconjecture]{conj:o-markov-equiv}
	Let $D_Y$ be a dataset for random vector $Y$ with superscript to index different datasets and size, i.e. $D_Y^{(1, n_{sample})}$ represent dataset 1 of $Y$ of $n_{sample}$ number of observations.
	Let $\mathbb{DAG}$ be the matrix group of DAGs (following other matrix group notations like $\mathbb{GL}$, $\mathbb{SO}(3)$, $\mathbb{SE}(3)$): $\mathbb{DAG}=\{W|W$~represents a DAG$\}$.

	Let $\mathcal{D}_{\epsilon}\in \mathbb{DI}_{|J|}$ be the set of idiosyncratic distributions for random vectors of idiosyncratic variable $\epsilon$ of size $|J|$, let $g$ denote a map, where
	\begin{align}
                &g:(\mathbb{DAG}, \mathbb{DI}_{|J_O|+|J_U|}) \nonumber\\& \to (\mathbb{DAG}, \mathbb{DI}_{|J_O|}, \mathbb{DI}_{|J_U|}) \\
		(W, \mathcal{D}_{\epsilon_Y})               & \mapsto \left(
		\begin{bmatrix}
			 & W_o & \Lambda \\  &0 &0
		\end{bmatrix}
		, {[\epsilon_O]}_{|J_O|\times 1} \sim \mathcal{D}_{\epsilon_O}, {[\xi]}_{|J_U|\times 1} \sim \mathcal{D}_{\xi}\right)
	\end{align}
	such that, when $\mathbb{DI}$ are mutually independent Gaussian, then
	\begin{align}
		\forall W & :=
		\begin{bmatrix}
			 & {[W]}_{J_O} & {[W]}_{J_{O}, J_{U}} \\  
                         &{[W]}_{J_{U}, J_{O}}\not\equiv {[0]}_{|J_U||J_O|} &{[W]}_{J_U} \not\equiv 0
		\end{bmatrix}
		\\
		          & =P_{|J_O|+|J_U|}L_{|J_O|+|J_U|}P_{|J_O|+|J_U|}^T
	\end{align}
	generate dataset ${D_Y}^{(1, n_{sample})}$ via idiosyncratic variable $\epsilon_Y$
	\begin{align}{D_Y}^{(1,  n_{sample})}(W, \epsilon_Y) & :=
             \begin{pmatrix}
		              & D_O^{(1,  n_{sample})} \\ &D_\xi^{(1,  n_{sample})}
	             \end{pmatrix}
             \sim \Cref{eq:yeqwy}~\text{with}~\epsilon_Y \sim \mathcal{D}_{\epsilon_Y}
	\end{align}
	then
	\begin{align}
          \exists &\left(W^{'}:=
		\begin{bmatrix}
			 & W_o & \Lambda \\  &0 &I
		\end{bmatrix}
		, {[\epsilon_O]}_{|J_O|\times 1} \sim \mathcal{D}_{\epsilon_O}, {[\xi]}_{|J_U|\times 1} \sim \mathcal{D}_{\xi}\right) \nonumber\\& =g(W, {[\epsilon_Y]}_{(|J_O|+|J_U|)\times 1} \sim \mathcal{D}_{\epsilon_Y})
	\end{align}
	where
	\begin{align}
		W_o & =P_{|J_O|}L_{|J_O|}P_{|J_O|}^T
	\end{align}
	sample $\Lambda$ following the constraint defined in~\Cref{eq:constraint_mat_Lambda},
	generate the second dataset $D_Y^{(2)}$ via mutually independent confounder $\xi$ and idiosyncratic variable $\epsilon_O$:
	\begin{align}
		D_{Y}^{(2,  n_{sample})}(W_o, \Lambda, \epsilon_O, \xi) & :=
		\begin{pmatrix}
			 & D_O^{(2,  n_{sample})} \\ &D_{\xi}^{(2,  n_{sample})}=\xi
		\end{pmatrix}
		\sim \Cref{eq:root_confounder_data_gen}                                                                                        \\
		s.t.                                                                                                                           \\
		CI(D_O^{(1,  n_{sample})})                              & =CI(D_O^{(2,  n_{sample})}),\text{when}~n_{sample}\rightarrow \infty
	\end{align}
	i.e., under such a transformation $g$, the corresponding marginal distribution of $O$ is Markov indistinguishable (the set of CI statements stay the same) given a dataset of $O$.
\end{myconjecture}

\begin{proof}
The special property of Gaussian distribution makes the covariance matrix of a marginal distribution just the block of the global covariant matrix, thus there are multiple possiblities for other blocks as long as p.s.d.~property is ensured.

According to the trek rule, the sub-block of the covariance matrix of the marginal distribution of $O$ has a contribution from the trek monimial topped at the root confounder $\xi$ with $\Lambda$ as the trek matrix.


Let the number of unobserved confounder to be $n_u$, then
$		W^{'}=\begin{bmatrix}
			 & W_o & \Lambda \\  &0 &0
		\end{bmatrix}
$ is at least $n_u$ rank deficient.

with $\Omega^{'}=diag(1)=I$

\begin{align}\label{eq:id_minus_w}
I-W^{'} &=   I- \begin{bmatrix}
		 & W_o & \Lambda \\
		 & 0   & I
	\end{bmatrix}\\
        &=\begin{bmatrix}
		 & I-W_o & I-\Lambda \\
		 & I   & 0
	\end{bmatrix}
\end{align}

\begin{align}\label{eq:id_minus_w}
{(I-W^{'})}^{-1} 	
        &={\begin{bmatrix}
		 & I-W_o & I-\Lambda \\
		 & I   & 0
        \end{bmatrix}}^{-1}
\end{align}

Take $\Omega^{'}=I$
\begin{align}
  \Sigma^{'}&=(I-W^{'})^{-1} \Omega^{'} {(I-W^{'})^{-1}}^T\\
            &=(I-W^{'})^{-1}{(I-W^{'})^{-1}}^T\\
            &={\begin{bmatrix}
		 & I-W_o & I-\Lambda \\
		 & I   & 0
        \end{bmatrix}}^{-1}
{\begin{bmatrix}
		 & I-W_o & I-\Lambda \\
		 & I   & 0
        \end{bmatrix}}^{-T}
\end{align}

\end{proof}

\begin{remark}
	However, even if there exist such a transformation, it does not necessarily mean it would be trivial to realize such an equivalent distribution in the state-of-the-art data synthesis protocol, as we analyzed in~\Cref{sec:dgp_old_admg_protocol}.
	In particular,~\Cref{conj:o-markov-equiv} only holds true at large sample limit.
	With finite sample sizes, it is difficult for the state-of-the-art method to cover the space our new synthesis protocol can cover.
\end{remark}
\begin{remark}
	When $\mathbb{DI}$ is not Gaussian, then~\Cref{conj:o-markov-equiv} does not necessarily hold true.
\end{remark}





==> z_obsolete_proof_connect_implicit_explicit.tex <==
Rewrite~\Cref{eq:root_confounder_data_gen}
\begin{align}
	Y^{'}:=
	\begin{pmatrix}
		 & Y_O   \\
		 & \xi
	\end{pmatrix}
	                                        & =
	\begin{bmatrix}
		 & W_o & \Lambda \\
		 & 0   & 0
	\end{bmatrix}
	\begin{pmatrix}
		 & Y_O   \\
		 & \xi
	\end{pmatrix}
	+
	\begin{pmatrix}
		 & \epsilon_O \\
		 & \xi
	\end{pmatrix}
	= W^{'}
	Y^{'}+\epsilon^{'}\\
&=TAT^{-1}Y^{'}+\epsilon^{'}\\
&\iff\nonumber\\
  T^{-1}Y^{'}&=AT^{-1}Y^{'}+T^{-1}\epsilon^{'}\\
&\iff\nonumber\\
Y^{''}&=AY^{''}+\epsilon^{''}
\end{align}

\begin{align}\label{eq:id_minus_w}
I-W^{'} &=   I- \begin{bmatrix}
		 & W_o & \Lambda \\
		 & 0   & I
	\end{bmatrix}\\
        &=\begin{bmatrix}
		 & I-W_o & I-\Lambda \\
		 & I   & 0
	\end{bmatrix}
\end{align}

\begin{align}\label{eq:id_minus_w}
{(I-W^{'})}^{-1} 	
        &={\begin{bmatrix}
		 & I-W_o & I-\Lambda \\
		 & I   & 0
        \end{bmatrix}}^{-1}
\end{align}


$\exists$ permutation matrix $E$ such that
\begin{align}
E \Omega E^T&=\begin{bmatrix}
     &L_1 & 0 \\
     & L_2   & 0
  \end{bmatrix}\\
  &\Omega=\begin{bmatrix}
     &L_1 & 0 \\
     & L_2   & 0
  \end{bmatrix}D\begin{bmatrix}
     &L_1 & 0 \\
     & L_2   & 0
  \end{bmatrix}
\end{align}



if the diagonal elements are distinct:
Via ($|\lambda_i(\Omega)-\lambda_i(diag(\Omega))|\le \frac{||E||^2}{\min_j|\lambda_i-\lambda_j|}$)~\citep{nakatsukasa2017off}, the spectral norm of the off-diagonal entries can be estimated, thus the number of off-diagonal entries could be estimated. 

If the diagonal elements are identical: with the help of the relation $\lambda_i(\Omega)=\lambda_i(diag(\Omega))+\frac{{v}^TEv}{v^Tv}+O(||E||^2)={[diag(\Omega)]}_i+\frac{{v}^TEv}{v^Tv}+O(||E||^2)$~\citep{nakatsukasa2017off}, where $v$ is the eigenvector of $diag(\Omega)$, i.e. the standard basis vector. When $v=(1,0, \ldots, 0)^T$, $\frac{{v}^TEv}{v^Tv}$ is zero. So we have to choose other basis as the eigenvector?\todo{This is not clear yet}
\end{conjecture}




==> z_proof.tex <==
%the covariance matrix of the variables after the transformation is ${Q}^{T}AQ$, the covariance matrix block ${\Sigma}_{11}$ of the variables is unchanged when using $A$ as adjacency matrix compared to using $W^{'}$ as adjacency matrix.
\begin{align}
&\mathbb{E}(Y_1^{''}{Y_1^{''}}^T)\nonumber\\
  =&\mathbb{E}[Y_O Y_O^T + Y_O \xi^T \Sigma_{12}^T \Sigma_{11}^{-T} + \Sigma_{11}^{-1}\Sigma_{12}\xi Y_O^T + \Sigma_{11}^{-1}\Sigma_{12}\xi \xi^T \Sigma_{12}^T \Sigma_{11}^{-T}]\\
  =&\Sigma_{11}+ 
 \Sigma_{12} \Sigma_{12}^T \Sigma_{11}^{-T} + \Sigma_{11}^{-1}\Sigma_{12}\Sigma_{12}^T + \Sigma_{11}^{-1}\Sigma_{12} \Sigma_{12}^T \Sigma_{11}^{-T}
\end{align}
Since
\begin{align}
\Sigma_{12}:=\mathbb{E}(Y_O \xi^T)&={(I-W_0)}^{-1}(\epsilon_O+\Lambda \xi)\xi^T\\
           &={(I-W_0)}^{-1}\Lambda
\end{align}

\begin{align}
\Sigma_{12}\Sigma_{12}^T={(I-W_0)}^{-1}\Lambda\Lambda^T{(I-W_0)}^{-T}
\end{align}

\begin{align}
\Sigma_{11}&:=
\mathbb{E}(Y_O{Y_O}^T)\nonumber\\
&={(I-W_0)}^{-1}(\epsilon_O+\Lambda \xi)(\epsilon_O^T+ \xi^T\Lambda^T) {(I-W_0)}^{-T}\\
             &={(I-W_0)}^{-1}(I+\Lambda\Lambda^T){(I-W_0)}^{-T}
\end{align}



